Scaling Team Coordination on Graphs with Reinforcement Learning

This paper studies Reinforcement Learning (RL) techniques to enable team coordination behaviors in graph environments with support actions among teammates to reduce the costs of traversing certain risky edges in a centralized manner. While classical approaches can solve this non-standard multi-agent path planning problem by converting the original Environment Graph (EG) into a Joint State Graph (JSG) to implicitly incorporate the support actions, those methods do not scale well to large graphs and teams. To address this curse of dimensionality, we propose to use RL to enable agents to learn such graph traversal and teammate supporting behaviors in a data-driven manner. Specifically, through a new formulation of the team coordination on graphs with risky edges problem into Markov Decision Processes (MDPs) with a novel state and action space, we investigate how RL can solve it in two paradigms: First, we use RL for a team of agents to learn how to coordinate and reach the goal with minimal cost on a single EG. We show that RL efficiently solves problems with up to 20/4 or 25/3 nodes/agents, using a fraction of the time needed for JSG to solve such complex problems; Second, we learn a general RL policy for any $N$-node EGs to produce efficient supporting behaviors. We present extensive experiments and compare our RL approaches against their classical counterparts.

==> Contents_abridged/results_abridged_backup.tex <==
\section{RESULTS}
\label{sec::results}

\begin{table*}[t]
\centering
\caption{Solution time for 2, 3, and 4 agents in JSG, Q-Learning and PPO respectively.}
\label{tab::time_comparison}
\small
\setlength{\tabcolsep}{2.5pt} % Default value: 6pt, 3pt
\begin{tabular}{ccccccccccc}
\toprule
Graph & Nodes & \multicolumn{3}{c}{2 Agents} & \multicolumn{3}{c}{3 Agents} & \multicolumn{3}{c}{4 Agents} \\
\cmidrule(rl){3-5} \cmidrule(rl){6-8} \cmidrule(rl){9-11} & & JSG & Q-Learning & PPO & JSG & Q-Learning & PPO & JSG & Q-Learning & PPO \\
\midrule
\multirow{5}{*}{Sparse} 
& 5  & \textbf{0.001} & 1.228 & 58.39 & \textbf{0.037} & 2.863 & 83.66 & \textbf{1.093} & 9.978 & 88.74 \\
& 10 & \textbf{0.014} & 3.654 & 81.39 & \textbf{1.494} & 10.35 & 226.2 & 157.7 & \textbf{102.7} & 355.8 \\
& 15 & \textbf{0.057} & 5.922 & 201.02 & \textbf{14.88} & 27.88 & 326.4 & 3652 & -- & \textbf{962.2} \\
& 20 & \textbf{0.172} & 13.86 & 560.3 & 80.16 & \textbf{45.31} & 701.5 & -- & -- & \textbf{1045} \\
& 25 & \textbf{0.394} & -- & 730.5 & \textbf{281.0} & -- & 1432 & -- & -- & -- \\
\midrule
\multirow{5}{*}{Moderate} 
& 5  & \textbf{0.002} & 0.293 & 56.97 & \textbf{0.052} & 3.469 & 74.03 & \textbf{1.689} & 14.34 & 88.21 \\
& 10 & \textbf{0.022} & 2.362 & 66.17 & \textbf{3.007} & 20.36 & 146.3 & 600.5 & 751.0 & \textbf{352.2} \\
& 15 & \textbf{0.088} & 2.389 & 189.6 & 25.49 & \textbf{22.79} & 317.7 & 9492 & -- & \textbf{949.4} \\
& 20 & \textbf{0.277} & 3.587 & 531.0 & 160.04 & \textbf{58.26} & 683.3 & -- & -- & \textbf{1032} \\
& 25 & \textbf{0.641} & 5.720 & 677.5 & 571.1 & \textbf{181.8} & 1372 & -- & -- & -- \\
\midrule
\multirow{5}{*}{Dense} 
& 5  & \textbf{0.002} & 0.874 & 57.32 & \textbf{0.072} & 1.855 & 72.44 & \textbf{0.072} & 6.921 & 89.71 \\
& 10 & \textbf{0.035} & 1.963 & 64.35 & \textbf{7.927} & 15.11 & 142.3 & 4312 & 696.9 & \textbf{344.8} \\
& 15 & \textbf{0.109} & 6.671 & 186.4 & \textbf{39.49} & 129.1 & 317.7 & 46455 & -- & \textbf{944.1} \\
& 20 & \textbf{0.433} & 2.616 & 646.2 & 481.4 & \textbf{65.22} & 677.5 & -- & -- & \textbf{1018} \\
& 25 & \textbf{0.915} & 5.192 & 700.9 & 1660 & 7821 & \textbf{1349} & -- & -- & --\\
\bottomrule
\end{tabular}
\vspace{-16pt}
\end{table*}

With our new problem formulation and implementation, we conduct extensive experiments to study how RL can efficiently enable team coordination on graphs with risky edges. We present experiment results of using RL to solve both single and multiple \textsc{eg}(s). 
% Although classical methods like \textsc{jsg} can already efficiently solve simple team coordination problems on graphs with a small amount of nodes and agents, we hypothesize that RL will be advantageous when facing complex problems with many nodes and agents. 

% Time compassion results for 2,3 and 4 agents can be found here\ref{tab:time_comparison}.
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/2_agents_sparse_new.png}
%     \caption{Pareto Plot Sparse 2 Agents}
%     \label{fig_wrt_riskedgratio}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/2_agents_moderate_new.png}
%     \caption{Pareto Plot Moderate 2 Agents}
%     \label{fig_wrt_riskedgratio}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/2_agents_dense_new.png}
%     \caption{Pareto Plot Dense 2 Agents}
%     \label{fig_wrt_riskedgratio}
% \end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/3_agents_sparse_new.png}
%     \caption{Pareto Plot Sparse 3 Agents}
%     \label{fig_wrt_riskedgratio}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/3_agents_moderate_new.png}
%     \caption{Pareto Plot Moderate 3 Agents}
%     \label{fig_wrt_riskedgratio}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/3_agents_dense_new.png}
%     \caption{Pareto Plot Moderate 3 Agents}
%     \label{fig_wrt_riskedgratio}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/4_agents_sparse_new.png}
%     \caption{Pareto Plot Sparse 4 Agents}
%     \label{fig_wrt_riskedgratio}
% \end{figure}
% \textcolor{red}{Manshi: I couldnt make 15 nodes comparsion and more for 4 agents for all JSG, Q-Learning and PPO.}














% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/pareto_plot_sparse_2agents.png}
%     \caption{Pareto Plot Sparse 2 Agents}
%     \label{fig_wrt_riskedgratio}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/pareto_plot_moderate_2agents.png}
%     \caption{Pareto Plot Moderate 2 Agents}
%     \label{fig_wrt_riskedgratio}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/pareto_plot_dense_2agents.png}
%     \caption{Pareto Plot Dense 2 Agents}
%     \label{fig_wrt_riskedgratio}
% \end{figure}



% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/pareto_plot_sparse_3agents.png}
%     \caption{Pareto Plot Sparse 3 Agents}
%     \label{fig_wrt_riskedgratio}
% \end{figure}


\subsection{RL for Single \textsc{eg}}
The first set of experiments is to use RL to solve one single \textsc{eg}. Despite that the classical \textsc{jsg} approach can be efficient in solving simple coordination problems on small graphs with a small number of agents, we hypothesize that RL has the potential to solve complex problems faster. Note that since \textsc{cjsg} can only address problems with up to two agents, and our goal is to extend to more than two, we do not include \textsc{cjsg} in our comparison. 

Specifically, we experiment with 5, 10, 15, 20, and 25 nodes with 2, 3, and 4 agents in three types of graph connectivity, i.e., sparse, moderate, and dense, using \textsc{jsg}, Q-Learning, and PPO. We randomly create 15 \textsc{eg}s as our test set. All experiment results are presented in Tab.~\ref{tab::time_comparison}. For both RL approaches, training is terminated when the cumulative reward no longer changes more than 0.2 for 500 steps. 

The results in Tab.~\ref{tab::time_comparison} shows that \textsc{jsg} outperforms both Q-Learning and PPO in all two-agent cases, indicating that the cost to construct a \textsc{jsg} for two agents and search on such a graph is minimal even with up to 25 nodes. However, RL's superiority starts to show when the number of agents and nodes and graph connectivity start to increase. For three agents, Q-Learning starts to outperform \textsc{jsg} in 20-node sparse graphs, while it completely overtakes \textsc{jsg} for moderate graphs with more than 15 nodes. Q-Learning and PPO outperform \textsc{jsg} on 20-node and 25-node dense graphs respectively. In most cases with four agents, PPO (and Q-Learning) is the fastest, except for small 5-node graphs. Notice that ``--'' denotes that the algorithm fails to find a solution, i.e., \textsc{jsg} runs out of memory during graph construction, Q-Learning's Q-table becomes intractably large, or PPO does not converge. All three methods fail to produce a solution for the most difficult case at the lower right of Tab.~\ref{tab::time_comparison}, i.e., four agents on 25-node dense graphs, while PPO is the only one that can solve for four agents on 20-node dense graphs. 


% \begin{table*}[t]
% \centering
% \caption{Time comparison for 2, 3, and 4 agents in JSG, Q-Learning and PPO respectively.\xuesu{Way too many digits. Leave only 3-4 digits is more than enough.}}
% \label{tab:time_comparison}
% \small
% \setlength{\tabcolsep}{2.5pt} % Default value: 6pt, 3pt
% \begin{tabular}{ccccccccccc}
% \toprule
% Graph & Nodes & \multicolumn{3}{c}{2 Agents} & \multicolumn{3}{c}{3 Agents} & \multicolumn{3}{c}{4 Agents} \\
% \cmidrule(rl){3-5} \cmidrule(rl){6-8} \cmidrule(rl){9-11} & & JSG & Q-Learning Mask & PPO Mask & JSG & Q-Learning Mask & PPO Mask & JSG & Q-Learning Mask & PPO Mask \\
% \midrule
% \multirow{5}{*}{Sparse} 
% & 5  & 0.0014 & 1.2276 & 58.386 & 0.0373 & 2.8628 & 83.655 & 1.0927 & 9.9784 & 88.736 \\
% & 10 & 0.0135 & 3.6544 & 81.391 & 1.4935 & 10.3501 & 226.162 & 157.657 & 102.7302 & 355.807 \\
% & 15 & 0.0569 & 5.9218 & 201.019 & 14.8758 & 27.8827 & 326.352 & 3652.149 & -- & 962.178 \\
% & 20 & 0.1715 & 13.8633 & 560.289 & 80.1585 & 45.3061 & 701.504 & -- & -- & 1045.320 \\
% & 25 & 0.3939 & -- & 730.545 & 280.982 & -- & 1431.670 & -- & -- & -- \\
% \midrule
% \multirow{5}{*}{Moderate} 
% & 5  & 0.0016 & 0.2932 & 56.971 & 0.05167 & 3.4688 & 74.034 & 1.6894 & 14.3405 & 88.212 \\
% & 10 & 0.0220 & 2.3622 & 66.170 & 3.00691 & 20.3604 & 146.258 & 600.508 & 750.9537 & 352.215 \\
% & 15 & 0.0880 & 2.3893 & 189.592 & 25.4882 & 22.7887 & 317.687 & 9491.781 & -- & 949.392 \\
% & 20 & 0.2766 & 3.5868 & 531.025 & 160.037 & 58.2607 & 683.281 & -- & -- & 1032.213 \\
% & 25 & 0.6411 & 5.7202 & 677.544 & 571.056 & 181.7779 & 1372.273 & -- & -- & -- \\
% \midrule
% \multirow{5}{*}{Dense} 
% & 5  & 0.00205 & 0.8743 & 57.324 & 0.07230 & 1.8552 & 72.445 & 0.07230 & 6.9214 & 89.709 \\
% & 10 & 0.03509 & 1.9634 & 64.352 & 7.92671 & 15.1146 & 142.275 & 4311.622 & 696.8927 & 344.815 \\
% & 15 & 0.10861 & 6.6710 & 186.425 & 39.4919 & 129.0906 & 317.689 & 46455.350 & -- & 944.133 \\
% & 20 & 0.43322 & 2.6163 & 646.192 & 481.441 & 65.2154 & 677.450 & -- & -- & 1018.041 \\
% & 25 & 0.91504 & 5.1919 & 700.893 & 1659.852 & 7820.6237 & 1348.986 & -- & -- & --\\
% \bottomrule
% \end{tabular}
% \end{table*}



For solving one \textsc{eg}, while RL cannot guarantee optimality, we observe that in most cases RL can achieve optimal solutions, and near-optimal ones in others. We use the four agents in 10- and 15-node graphs as an example and present the optimality vs. time plots in Fig.~\ref{fig::pareto_1st_half}. We also implement a naive approach, in which all agents do not seek coordination, but just move towards the goals with the minimal cost paths. The naive approach is very efficient in terms of time, since it only needs to call a shortest-path algorithm on the \textsc{eg}, but without coordination the naive approach will incur a large cost. On the other hand, \textsc{jsg} is provably optimal~\cite{limbu2023team}, so we use the ratio between the optimal \textsc{jsg} cost and a solution's cost as an indication of solution optimality. In Fig.~\ref{fig::pareto_1st_half}, the horizontal axis is the reciprocal of the solution time in log scale, while the vertical axis is the optimality value between 0 and 1. Naive approach is expected to appear in the lower right corner by achieving very short solution time but very low path quality, whereas \textsc{jsg} should be in the upper left corner with optimality value 1 and a very long solution time. 
For four agents on sparse 10-node graphs, PPO does not produce any advantage over \textsc{jsg}, by achieving lower optimality with longer time. But for sparse 15-node graphs, PPO outperforms \textsc{jsg} by achieving optimality with better time efficiency. For moderate 10- and 15-node graphs, PPO achieves a middle ground in terms of both optimality and time between \textsc{jsg} and the naive approach. We observe the same optimality-time trend in dense graphs of 10 and 15 nodes. In all scenarios, the worst optimality ratio PPO can achieve is more than 70\% of \textsc{jsg}'s absolute optimality value, but mostly with better time efficiency than \textsc{jsg}. 

   % \includegraphics[width=0.32\textwidth]{figures/4_agents_sparse_final_sparse.png}
   %  \includegraphics[width=0.32\textwidth]{figures/4_agents_sparse_final_moderate.png}
   %  \includegraphics[width=0.32\textwidth]{figures/4_agents_sparse_final_dense.png}

\begin{figure*}
    \centering
    \includegraphics[width=0.32\textwidth]{figures/final_4_agents_sparse.png}
    \includegraphics[width=0.32\textwidth]{figures/final_4_agents_moderate.png}
    \includegraphics[width=0.32\textwidth]{figures/final_4_agents_dense.png}
    \caption{Single \textsc{eg}: Optimality vs. Time plots for four agents on sparse, moderate, and dense graphs. }
    \label{fig::pareto_1st_half}
    \vspace{-10pt}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=0.32\textwidth]{figures/2nd_half_5_nodes.png}
    \includegraphics[width=0.32\textwidth]{figures/2nd_half_10_nodes_gridstyle_graph.png}
    \caption{Multiple \textsc{eg}: Optimality vs. Time plots for two agents on any 5- or 10-node graphs. }
    \label{fig::pareto_2nd_half}
    \vspace{-16pt}
\end{figure*}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/4_agents_sparse_final_sparse.png}
%     \caption{\textcolor{red}{1st half} Pareto Plot for 4 agents in Sparse Graph.}
%     \label{fig_pareto_4_sparse}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/4_agents_sparse_final_moderate.png}
%     \caption{\textcolor{red}{1st half} Pareto Plot for 4 agents in Moderate Graph.}
%     \label{fig_pareto_4_moderate}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/4_agents_sparse_final_dense.png}
%     \caption{\textcolor{red}{1st half} Pareto Plot for 4 agents in Dense Graph.}
%     \label{fig_pareto_4_moderate}
% \end{figure}


\subsection{RL for Multiple \textsc{eg}}

The second set of experiments is to use RL to solve any $N$-node graphs. This is a very difficult task considering the variations in graph connectivities and supporting mechanisms with a large number of nodes. Therefore, we only limit our experiments within up to 10 nodes and 2 agents and leave extending to more complex problems to future work, potentially with decentralized approaches. Notice that when RL converges to a good policy, despite the long time it may require, this policy can then be used as an available tool to solve any team coordination problem on any $N$-node graph in the future. In the second set of experiments, training usually takes hours, which is considered as a one-time cost. Once trained, we compare RL's inference time and optimality of solving any $N$-node graph with \textsc{jsg} and the naive approach, as shown in Fig.~\ref{fig::pareto_2nd_half}. Q-Learning does not scale well to this challenging problem by underperforming \textsc{jsg} in terms of both optimality and time, while PPO can find the middle ground in terms of optimality and time between \textsc{jsg} and the naive approach. The PPO results (magenta crosses) in both graphs indicate that for any 5-node and 10-node graph, on average PPO can solve it with 70\% and 80\% optimality and half of the time compared to \textsc{jsg} respectively. 


